Spatial mixing and approximate counting for Potts model on graphs with bounded average degree

We propose a notion of contraction function for a family of graphs and establish its connection to the strong spatial mixing for spin systems. More specifically, we show that for anti-ferromagnetic Potts model on families of graphs characterized by a specific contraction function, the model exhibits strong spatial mixing, and if further the graphs exhibit certain local sparsity which are very natural and easy to satisfy by typical sparse graphs, then we also have FPTAS for computing the partition function. This new characterization of strong spatial mixing of multi-spin system does not require maximum degree of the graphs to be bounded, but instead it relates the decay of correlation of the model to a notion of effective average degree measured by the contraction of a function on the family of graphs. It also generalizes other notion of effective average degree which may determine the strong spatial mixing, such as the connective constant, whose connection to strong spatial mixing is only known for very simple models and is not extendable to general spin systems. As direct consequences: (1) we obtain FPTAS for the partition function of $q$-state anti-ferromagnetic Potts model with activity $0\le\beta<1$ on graphs of maximum degree bounded by $d$ when $q> 3(1-\beta)d+1$, improving the previous best bound $\beta> 3(1-\beta)d$ and asymptotically approaching the inapproximability threshold $q=(1-\beta)d$, and (2) we obtain an efficient sampler (in the same sense of fully polynomial-time almost uniform sampler, FPAUS) for the Potts model on Erd\H{o}s-R\'enyi random graph $\mathcal{G}(n,d/n)$ with sufficiently large constant $d$, provided that $q> 3(1-\beta)d+4$. In particular when $\beta=0$, the sampler becomes an FPAUS for for proper $q$-coloring in $\mathcal{G}(n,d/n)$ with $q> 3d+4$, improving the current best bound $q> 5.5d$ for FPAUS for $q$-coloring in $\mathcal{G}(n,d/n)$.

==> coloring.tex <==
\section{$\beta=0$ (Coloring model)}

In this section, we consider the coloring model, i.e., the Potts model
when $\beta=0$. In this model, some configurations become infeasible,
and we need some more effort to deal with them.

\subsection{Definitions}

In coloring model, pinning some vertex $v$ with color $x$ is
equivalent to removing the color from the available list of colors of
all its neighbors. Sometimes it is more convenient to state our
results in terms of \emph{list-colorings}.

Let $G=(V,E)$ be a graph, $q>0$ be an integer.. A \emph{list-coloring}
instance is a pair $(G,\mathcal{L})$ where
$\mathcal{L}=\langle L(v) : v\in V\rangle$ such that each
$L(v)\subseteq[q]$ specifies a list of colors for vertex $v$. A proper
coloring of $(G,\mathcal{L})$ is a assignment $\sigma:V\to [q]$ of
colors to vertices such that $\sigma(v)\in L(v)$ and
$\sigma(u)\ne\sigma(v)$ for every $(u,v)\in E$.  A list-coloring
instance $(G,\mathcal{L})$ is \emph{feasible} if a proper coloring
$\sigma$ exists. In the case that $L(v)=[q]$ for every $v\in V$,
$(G,\mathcal{L})$ is an instance of $q$-coloring and we write it as
$(G,[q])$.

\begin{definition}
  Given a list-coloring instance $(G,\mathcal{L})$, a vertex $v$ is
  said to be \emph{permissive} if for all neighbors $u$ of $v$ and
  $u=v$, it holds that $|L(u)|\ge\deg[G]{u}+3$.
  % A set $S$ of vertices is said to be permissive if all vertices in
  % $S$ are permissive.
\end{definition}

Note that by above definition, a vertex $v$ is permissive if only if
itself and all its neighbors are soft.

We have defined the notion of soft cutset in Potts model. However, in
coloring model, a stronger notion turns out to be necessary:

\begin{definition}
  Let $(G,\mathcal{L})$ be a list-coloring instance, $G=(V,E)$ and
  $v\in V$. Let $T=\Tsaw{G}{v}$ and $\Delta\subseteq V(T)$ be a set of
  vertices in $T$. A set $S$ of vertices in $T$ is called a
  \emph{permissive cutset} for $v$ and $\Delta$ in $T$, if it holds
  that (1) every self-avoiding walk from $v$ to $\Delta$ intersect
  with $S$ and (2) every vertex in $S$ is identified to a permissive
  verteix in $G$ by $\Tsaw{G}{v}$.
\end{definition}

\begin{definition}
  Let $(G,\mathcal{L})$ be a list-coloring instance, $G=(V,E)$ and
  $v\in V$. Let $T=\Tsaw{G}{v}$. A set of vertices $S$ in $T$ is
  called \emph{permissive $\ell$-cutset}, if: (1) the depths of all
  vertices in $S$ are in $[\ell,2\ell)$; (2) every self-avoiding walk
  from $v$ of length $\ge 2\ell$ must intersect with $S$ in $T$; and
  (3) every vertex in $S$ is identified to a permissive vertex in $G$
  by $\Tsaw{G}{v}$.
\end{definition}

Unlike the Potts model, the feasibility of a configuration is a big
issue. Let $(G(V,E),\mathcal{L})$ be a feasible instance of
list-coloring with $L(v)\subseteq [q]$ for all $v\in V$.  Let
$S\subseteq V$ and $(G[S],\mathcal{L}_S)$ be the instance where
$\mathcal{L}_S=\set{L(v)\mid v\in S}$. A coloring $\sigma:S\to[q]$ is
called (globally) feasible if there exists a proper coloring
$\pi:V\to[q]$ of $(G,\mathcal{L})$ such that $\rho$ and $\pi$ are
consistent on $S$. We use $L(S)$ to denote the set of all such
feasible colorings. A coloring $\sigma:S\to[q]$ is called
\emph{locally feasible} if it is a proper coloring of
$(G[S],\mathcal{L}_S)$.

For permissive blocks, local feasibility implies global feasibility.

\begin{proposition}\label{prop:local-feasibility}
  Let $(G(V,E),\mathcal{L})$ be a feasible list-coloring instance. Let
  $B\subseteq V$ be a permissive block and $\pi$ be a locally feasible
  coloring on $B$. Then $\pi$ is feasible, i.e., $\pi\in L(B)$.
  % Define the instance $(G_\pi,\mathcal{L}_{\pi})$ as $G_{\pi}\defeq
  % G[V\setminus S]$,
  % $L_\pi(u)=L(u)$ for all $u\not\in\partial S$ and
  % $L_\pi(u)=L(u)\setminus \set{\pi(v)\mid v\in S\mbox{ and }
  % (v,u)\in
  % E}$. Then $(G_\pi,\mathcal{L}_\pi)$ is also feasible.
\end{proposition}
\begin{proof}
  Consider the instance $(G',\mathcal{L}')$ where $G'=G[V\setminus B]$
  and $\mathcal{L}'=\set{L'(v)\mid v\in V\setminus B}$ such that
  $L'(v)=L(v)$ for all $v\not\in\partial B$ and
  $L'(v)=L(v)\setminus\set{\pi(u)\mid (u,v)\in E}$ for all
  $v\in \partial B$. This instance is equivalent to the instance of
  $(G,\mathcal{L})$ after pinning $S$ with coloring $\pi$.  Since
  $(G,\mathcal{L})$ is feasible, there is a proper coloring for
  $G[V\setminus\tuple{B\cup\partial B}]$.  By our construction, it is
  clear that for every $v\in \partial B$,
  $\abs{L'(v)}-\deg[G']{v}\ge \abs{L(v)}-\deg[G]{v}$. We can therefore
  extend $\sigma$ to a proper coloring of $(G',\mathcal{L}')$ in a
  greedy fashion and this proves that $\pi$ is feasible.
\end{proof}
With this proposition, we do not distinguish between locally and
globally feasible colorings of a permissive block, and we just refer
them as proper colorings of $B$.


% Thus our estimation algorithm can be stated in terms of
% list-coloring.\todo{change the def of
% $\mathcal{E}_{\delta_{q,\beta},L}$}




\subsection{Strong spatial mixing}

Lemma \ref{thm:ssm} does not hold in general when $\beta=0$, we need
some additional condition to establish the strong spatial mixing
property for coloring model.

\begin{theorem}\label{thm:ssm-color}
  Let $q\ge 2$ be an integer.  Define a function
  $\delta_{q,\beta}:\mathbb{N}\to\mathbb{R}^+$ as
  \[
    \delta_{q,\beta}(x)=
    \begin{cases}
      \frac{2}{q-x-1}&\mbox{if }x\le q-3\\
      1 & \mbox{otherwise.}
    \end{cases}
  \]
  There exist two constant $C_1,C_2>0$ such that for every
  $G(V,E)\in \mathcal{G}_{\delta_{q,\beta}}$, every vertex $v\in V$,
  every color $x\in[q]$ and every set of vertices
  $\Lambda\subseteq V\setminus\set{v}$, if there exists a permissive
  cutset $S_v$ for $v$ and $\Delta\subseteq \Lambda$ in
  $T=\Tsaw{G}{v}$, then it holds that
  \[
    \abs{\Pr[G]{c(v)=x\mid c(\Lambda)=\rho}-\Pr[G]{c(v)=x\mid
        c(\Lambda)=\pi}}\le C_1\cdot\exp{-C_2\cdot\ell},
  \]
  where $\rho,\pi\in [q]^\Lambda$ are two feasible coloring of
  $\Lambda$ that differ on $\Delta$ and $\ell=\dist[T]{v,S_v}$.
\end{theorem}
\begin{proof}
  Let $T_v=\Tsaw{G}{v}$ and $S_v$ be the permissive cutset guaranteed
  by the premise of the theorem. Recursively define the error function
  $\mathcal{E}_{T_v,\delta,S}$:
  \[
    \mathcal{E}_{T_v,\delta,S}\defeq
    \begin{cases}
      \sum_{i\in[d]}
      \delta_{q,\beta}(\deg[G]{v_i})\cdot\mathcal{E}_{T_{v_i},S}&
      \mbox{if
      }v\not\in S\\
      3q &\mbox{otherwise.}
    \end{cases}
  \]
  Then we have the following analogue of Lemma \ref{lem:boundforS}:
  There exist two constants $C_1,C_2>0$ such that
  \[
    \mathcal{E}_{T_v,\delta_{q,\beta},S_v}\le
    C_1\cdot\exp{-C_2\cdot\ell}.
  \]
  The remaining proof is almost identical to the proof of Theorem
  \ref{thm:ssm}.
\end{proof}


\subsection{Sampling algorithm}


\begin{theorem}
  Let $q>1$ be an integer and $\beta=0$. Let $\mathcal{G}$ be a family
  of graphs. Assume there exists a constant $C>0$ such that for every
  $\ell(n)\ge C\log n$, every graph $G(V,E)\in\mathcal{G}$ with
  $\abs{V}=n$ and every $v\in V$, it holds that
  \begin{enumerate}
  \item
    $\sum_{L=\ell(n)}^{2\ell(n)}\mathcal{E}_{\delta_{q,\beta},L}\le
    n^{C_1}\cdot\exp{-C_2\cdot\ell(n)}$
    where $C_1,C_2>0$ are two universal constants;
  \item there exists an $\ell(n)$-permissive cutset $S_v$ in $T=\Tsaw{G}{v}$;%  such
    % that $\ell(n)\le \dist[T]{v,u}\le 2\ell(n)$;
  \item $\tau_{\ell(n)}(v)=2^{O(\ell(n))}$.
  \end{enumerate}
  Then for every $G(V,E)\in\mathcal{G}$ with $\abs{V}=n$, every
  $v\in V$ and every $x\in[q]$, the above algorithm computes
  $\hat p_{\Omega,v,S_v}(x)=\mathtt{marg}(\Omega,S_v,v,x)$ in time
  polynomial in $n$, satisfying
  \[
    1-O\tuple{\frac{1}{n^3}}\le \frac{\hat
      p_{\Omega,v,S_v}(x)}{\Pr[\Omega]{c(v)=x}} \le
    1+O\tuple{\frac{1}{n^3}},
  \]
  where $\Omega=(G,R,\sigma)$ is a \emph{feasible} coloring instance.
\end{theorem}
\begin{proof}
  The proof of this theorem is almost identical to the proof of
  Theorem \ref{thm:comp-marg}, except here $S_v$ are permissive
  cutset.
\end{proof}


\begin{theorem}\label{thm:list-coloring-marg}
  Let $q>1$ be an integer and $\mathcal{G}$ be a family of
  graphs. Assume there exists a constant $C>0$ such that for every
  $\ell(n)\ge C\log n$, every graph $G(V,E)\in\mathcal{G}$ with
  $\abs{V}=n$ and every $v\in V$, it holds that
  \begin{enumerate}
  \item
    $\sum_{L=\ell(n)}^{2\ell(n)}\mathcal{E}_{\delta_{q,\beta},L}\le
    n^{C_1}\cdot\exp{-C_2\cdot\ell(n)}$
    where $C_1,C_2>0$ are two universal constants;
  \item there exists a permissive cutset $S_v$ in $T=\Tsaw{G}{v}$ such
    that $\ell(n)\le \dist[T]{v,u}\le 2\ell(n)$;
  \item $\tau_{\ell(n)}(v)=2^{O(\ell(n))}$.
  \end{enumerate}
  Then for every $G(V,E)\in\mathcal{G}$ with $\abs{V}=n$, every
  $v\in V$ and every $x\in[q]$, there exists an algorithm to compute
  $\hat p_{(G,\mathcal{L}),v,S_v}(x)$ in time polynomial in $n$,
  satisfying
  \[
    1-O\tuple{\frac{1}{n^3}}\le \frac{\hat
      p_{(G,\mathcal{L}),v,S_v}(x)}{\Pr[G,\mathcal{L}]{c(v)=x}} \le
    1+O\tuple{\frac{1}{n^3}},
  \]
  where $(G,\mathcal{L})$ is a \emph{feasible} instance of
  list-coloring.
\end{theorem}


\begin{theorem}
  Let $\mathcal{G}$ be a family of graphs satisfying the conditions in
  Theorem \ref{thm:list-coloring-marg}. There exists an FPTAS to
  compute the partition function of feasible instance
  $(G,\mathcal{L})$ for every graph in $\mathcal{G}$.
\end{theorem}

\begin{corollary}
  There exists an FPAUS for list-coloring for a family of graphs
  satisfying conditions in Theorem \ref{thm:list-coloring-marg}.
\end{corollary}

